Discovery and Characterization of an Eccentric, Warm Saturn Transiting the Solar Analog TOI-4994

We present the detection and characterization of TOI-4994b (TIC 277128619b), a warm Saturn-sized planet discovered by the NASA Transiting Exoplanet Survey Satellite (TESS). TOI-4994b transits a G-type star (V = 12.6 mag) with a mass, radius, and effective temperature of $M_{\star} =1.005^{+0.064}_{-0.061} M_{\odot}$, $R_{\star} = 1.055^{+0.040}_{-0.037} R_{\odot}$, and $T_{\rm eff} = 5640 \pm 110$ K. We obtained follow-up ground-based photometry from the Las Cumbres Observatory (LCO) and the Antarctic Search for Transiting ExoPlanets (ASTEP) telescopes, and we confirmed the planetary nature of TOI-4994b with multiple radial velocity observations from the PFS, CHIRON, HARPS, FEROS, and CORALIE instruments. From a global fit to the photometry and radial velocities, we determine that TOI-4994b is in a 21.5-day, eccentric orbit ($e = 0.32 \pm 0.04$) and has a mass of $M_{P}= 0.280^{+0.037}_{-0.034} M_{J}$, a radius of $R_{P}= 0.762^{+0.030}_{-0.027}R_{J}$, and a Saturn-like bulk density of $\rho_{p} = 0.78^{+0.16}_{-0.14}$ $\rm g/cm^3$. We find that TOI-4994 is a potentially viable candidate for follow-up stellar obliquity measurements. TOI-4994b joins the small sample of warm Saturn analogs and thus sheds light on our understanding of these rare and unique worlds.

==> EXOFAST_Stellar.tex <==
\begin{table}
\scriptsize
\centering
\caption{Median values and 68\% confidence interval for global model of TOI-4994.}
\begin{tabular}{lcccc}
  \hline
  \hline
\textbf{Parameter} & \textbf{Values} & & & \\
\hline
%\multicolumn{2}{l}{Stellar Parameters:}&\smallskip\\
Mass (\msun) &$1.005^{+0.064}_{-0.061}$\\
Radius (\rsun) &$1.055^{+0.04}_{-0.037}$\\
Luminosity (\lsun) &$1.02^{+0.041}_{-0.052}$\\
Density (cgs) &$1.21^{+0.17}_{-0.16}$\\
Surface gravity (cgs) &$4.393^{+0.045}_{-0.046}$\\
Effective Temperature (K) &5640 $\pm$ 110 \\
$\rm [Fe/H]$ Metallicity (dex) & $0.165^{+0.083}_{-0.084}$\\
Initial Metallicity  &$0.176^{+0.079}_{-0.08}$\\
Age (Gyr) &$6.3^{+4.2}_{-3.8}$\\
Equal Evolutionary Point &$380^{+31}_{-41}$\\
%~~~~$vsinI_*$\dotfill &Projected rotational velocity (km/s)\dotfill &$19.76\pm0.160$\\
%~~~~$\xi$\dotfill &Macroturbulence velocity (km/s)\dotfill &$5.76^{+0.51}_{-0.50}$\\
\hline
\end{tabular}
\begin{flushleft} 
  \footnotesize{ 
    \textbf{\textsc{NOTES:}}
$^\dagger$The initial metallicity is the metallicity of the star when it was formed. $^\ddagger$The Equal Evolutionary Point corresponds to static points in a stars evolutionary history when using the MIST isochrones and can be a proxy for age. See \S2 in \citet{Dotter:2016} for a more detailed description of EEP.
               }
 \end{flushleft}
\label{tab:exofast_stellar}
\end{table}
